Which anonymization technique is best for which NLP task? -- It depends. A Systematic Study on Clinical Text Processing

Clinical text processing has gained more and more attention in recent years. The access to sensitive patient data, on the other hand, is still a big challenge, as text cannot be shared without legal hurdles and without removing personal information. There are many techniques to modify or remove patient related information, each with different strengths. This paper investigates the influence of different anonymization techniques on the performance of ML models using multiple datasets corresponding to five different NLP tasks. Several learnings and recommendations are presented. This work confirms that particularly stronger anonymization techniques lead to a significant drop of performance. In addition to that, most of the presented techniques are not secure against a re-identification attack based on similarity search.

==> final_tables.tex <==

\begin{table*}[h!]
\centering
\small
\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c |}
\hline

{} &         De-ident &      Mask\_Nr &     Shuffle &      RS 20\% &      SS 20\% &      RS 100\% &      SS 100\%  &        CCSR &        Agg 2 &        Agg 3 &        Agg 4 \\
\hline

smoking &  +2.22\% (d) &  +1.06\% (d) &  +1.84\% (d) &  -4.34\% (d) &   -4.0\% (d) &  -10.46\% (d) &  -14.07\% (d)  &   +1.0\% (d) &   -5.61\% (d) &   -6.07\% (d) &   -6.53\% (d) \\
obesity &   +0.8\% (d) &  -0.61\% (d) &  -2.55\% (d) &  -1.94\% (d) &  -2.99\% (d) &   +1.96\% (d) &   -3.45\% (d)  &  -1.31\% (d) &  -12.48\% (d) &  -22.59\% (d) &  -36.97\% (d) \\
mednli  &  +1.55\% (c) &  +0.14\% (c) &           - &  -1.13\% (c) &  -2.52\% (c) &   -1.93\% (c) &   -8.42\% (c)  &  -0.73\% (c) &   -7.98\% (c) &  -13.34\% (c) &  -14.81\% (c) \\
clinsts &  -1.21\% (c) &  -0.12\% (c) &           - &  -1.36\% (c) &  -1.92\% (c) &   -0.95\% (c) &  -21.96\% (c)  &  -1.84\% (c) &    -3.3\% (c) &   -7.26\% (c) &  -24.31\% (c) \\
2010    &  -0.83\% (c) &   -5.1\% (c) &           - &  -3.04\% (c) &  -2.73\% (c) &  -25.12\% (c) &   -9.72\% (c)  &  -1.19\% (c) &            - &            - &            - \\
2018    &  -0.32\% (c) &   -0.5\% (c) &           - &  -4.34\% (c) &  -5.96\% (c) &  -16.94\% (c) &  -15.77\% (c)  &  -2.48\% (c) &            - &            - &            - \\
\hline
mean    &     +0.368\% &     -0.855\% &     -0.355\% &     -2.692\% &     -3.353\% &      -8.907\% &     -12.232\%  &     -1.092\% &      -7.342\% &     -12.315\% &     -20.655\% \\
\hline

\end{tabular}
\caption{Anonymization Effects.}
\label{table: Anonymization Effects.}  
\end{table*}


==> tables.tex <==

\begin{table}[h!]
\centering
\begin{tabular}{| p{1cm} | p{1.2cm} | p{1.2cm} | p{1.2cm} | p{1.2cm} | p{1.2cm} | p{1.2cm} |}
\hline
{} & mednli & clinsts &   2010 &   2018 & smoking & obesity \\
\hline
b &   76.9 &   83.88 &  82.62 &  87.84 &   77.89 &   67.58 \\
c &  80.49 &   84.83 &  84.54 &  89.03 &   75.48 &   70.73 \\
d &      - &       - &      - &      - &   87.01 &   82.51 \\
\hline
\end{tabular}
\caption{Benchmark Results.}
\label{table: Benchmark Results}  
\end{table}


\begin{table}[h!]
\centering
\begin{tabular}{| p{2cm} | p{2.5cm} | p{2.5cm} | p{2.5cm} |}
\hline
{} & Dei &    Mask\_n &     Shuffle \\
\hline
smoking &        +2.22\% (d) &  +1.06\% (d) &  +1.84\% (d) \\
obesity &         +0.8\% (d) &  +0.52\% (b) &  -2.55\% (d) \\
mednli  &        +1.55\% (c) &  +0.14\% (c) &           - \\
clinsts &        -1.21\% (c) &  -0.12\% (c) &           - \\
2010    &        -0.33\% (b) &   -4.3\% (b) &           - \\
2018    &        +0.18\% (b) &  -0.47\% (b) &           - \\
\hline
mean    &           +0.535\% &     -0.528\% &     -0.355\% \\
\hline
\end{tabular}
\caption{Anonymization Effects.}
\label{table: Anonymization Effects.}  
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{| p{2cm} | p{2.5cm} | p{2.5cm} | p{2.5cm} |}
\hline
{} &      RS 20\% &      SR 20\% &        CCSR \\
\hline
smoking &  -4.34\% (d) &   -4.0\% (d) &   +1.0\% (d) \\
obesity &  -1.94\% (d) &  -2.99\% (d) &  -1.31\% (d) \\
mednli  &  -1.13\% (c) &  -2.52\% (c) &  -0.73\% (c) \\
clinsts &  -0.93\% (b) &  -1.92\% (c) &  -1.43\% (b) \\
2010    &  -3.03\% (b) &   -2.6\% (b) &  -1.19\% (c) \\
2018    &  -4.34\% (c) &  -5.96\% (c) &  -2.48\% (c) \\
\hline
mean    &     -2.618\% &     -3.332\% &     -1.023\% \\
\hline
\end{tabular}
\caption{Anonymization Effects.}
\label{table: Anonymization Effects.}  
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{| p{2cm} | p{2.5cm} | p{2.5cm} | p{2.5cm} |}
\hline
{} &        Agg 2 &        Agg 3 &        Agg 4 \\
\hline
smoking &   -5.61\% (d) &   -6.07\% (d) &   -6.53\% (d) \\
obesity &  -12.48\% (d) &  -18.64\% (b) &  -20.45\% (b) \\
mednli  &   -7.98\% (c) &   -12.6\% (b) &  -14.81\% (c) \\
clinsts &    -1.3\% (b) &   -7.26\% (c) &   -16.4\% (b) \\
2010    &            - &            - &            - \\
2018    &            - &            - &            - \\
\hline
mean    &      -6.842\% &     -11.142\% &     -14.548\% \\
\hline
\end{tabular}
\caption{Anonymization Effects.}
\label{table: Anonymization Effects.}  
\end{table}




\begin{table}[H]
\centering
\small
\begin{tabular}{|p{0.12\textwidth}||p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}|p{0.13\textwidth}|p{0.13\textwidth}|}
\hline 
 Corpus & Smoking & Obesity & 2010NER & 2018NER & MedNLI & ClinSTS \\
\hline 
\hline 
 NLP Task & MCC & MLC & NER & NER & NLI & STS \\
\hline 
 Train size & 389 & 730 & 170 & 303 & 11232 & 1642 \\
\hline 
 Dev size & 104* & 507* & 256* & 202* & 1395 & 412* \\
\hline 
 Test size & 104 & 507 & 256 & 202 & 1422 & 412 \\
\hline 
 Text type & discharge & discharge & discharge & discharge & sent. pairs & sent. pairs \\
\hline 
 Avg token & 1100.61 & 1935.72  & 15.41 & 63.657 & 37.22 & 57.65 \\
%\hline 
% Min, Max token length & 155,3998 & 275, 6852 & 1, 486 & 1, 179 & 9, 389 & 21, 280 \\
 \hline 
 %Source & \cite{2006} & \cite{2008} & \cite{2010} & \cite{2018} & [] & \cite{clinsts} \\
 %\hline
\end{tabular}
\caption{Overview about the different datasets used, including their underlying tasks, such as MCC (multi-class classification), MLC (multi-label classification), NER (named entity recognition), NLI (natural language inference and STS (sentence similarity). In case of * no development (dev) set was provided, the test set was used instead.}
\label{table:Datasets overview}     
\end{table}



==> tables2.tex <==
\newpage



\begin{table}[h!]
\centering
\begin{tabular}{| p{1cm} | p{1.2cm} | p{1.2cm} | p{1.2cm} | p{1.2cm} | p{1.2cm} | p{1.2cm} |}
\hline
{} & mednli & clinsts &   2010 &   2018 & smoking & obesity \\
\hline
b &   76.9 &   83.88 &  82.62 &  87.84 &   77.89 &   67.58 \\
c &  80.49 &   84.83 &  84.54 &  89.03 &   75.48 &   70.73 \\
d &      - &       - &      - &      - &   87.01 &   82.51 \\
\hline
\end{tabular}
\caption{Benchmark Results.}
\label{table: Benchmark Results}  
\end{table}




\begin{table}[h!]
\centering
\begin{tabular}{| p{2cm} | p{2.5cm} | p{2.5cm} | p{2.5cm} |}
\hline

{} &         Dei &      Mask\_n &     Shuffle \\
\hline

smoking &  +2.22\% (d) &  +1.06\% (d) &  +1.84\% (d) \\
obesity &   +0.8\% (d) &  -0.61\% (d) &  -2.55\% (d) \\
mednli  &  +1.55\% (c) &  +0.14\% (c) &           - \\
clinsts &  -1.21\% (c) &  -0.12\% (c) &           - \\
2010    &  -0.83\% (c) &   -5.1\% (c) &           - \\
2018    &  -0.32\% (c) &   -0.5\% (c) &           - \\
\hline
mean    &     +0.368\% &     -0.855\% &     -0.355\% \\
\hline

\end{tabular}
\caption{Anonymization Effects.}
\label{table: Anonymization Effects.}  
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{| p{2cm} | p{2.5cm} | p{2.5cm} | p{2.5cm} |}
\hline

{} &      RS 20\% &      SS 20\% &        CCSR \\
\hline

smoking &  -4.34\% (d) &   -4.0\% (d) &   +1.0\% (d) \\
obesity &  -1.94\% (d) &  -2.99\% (d) &  -1.31\% (d) \\
mednli  &  -1.13\% (c) &  -2.52\% (c) &  -0.73\% (c) \\
clinsts &  -1.36\% (c) &  -1.92\% (c) &  -1.84\% (c) \\
2010    &  -3.04\% (c) &  -2.73\% (c) &  -1.19\% (c) \\
2018    &  -4.34\% (c) &  -5.96\% (c) &  -2.48\% (c) \\
\hline
mean    &     -2.692\% &     -3.353\% &     -1.092\% \\
\hline

\end{tabular}
\caption{Anonymization Effects.}
\label{table: Anonymization Effects.}  
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{| p{2cm} | p{2.5cm} | p{2.5cm} | p{2.5cm} |}
\hline

{} &        Agg 2 &        Agg 3 &        Agg 4 \\
\hline

smoking &   -5.61\% (d) &   -6.07\% (d) &   -6.53\% (d) \\
obesity &  -12.48\% (d) &  -22.59\% (d) &  -36.97\% (d) \\
mednli  &   -7.98\% (c) &  -13.34\% (c) &  -14.81\% (c) \\
clinsts &    -3.3\% (c) &   -7.26\% (c) &  -24.31\% (c) \\
2010    &            - &            - &            - \\
2018    &            - &            - &            - \\
\hline
mean    &      -7.342\% &     -12.315\% &     -20.655\% \\
\hline

\end{tabular}
\caption{Anonymization Effects.}
\label{table: Anonymization Effects.}  
\end{table}








\begin{table}[h!]
\centering
\begin{tabular}{| p{4cm} | p{2cm} | p{2cm} | p{2cm} |}

\hline

{} &     Dei &  Mask\_n & Shuffle \\
\hline

words               &     1.0 &     1.0 &     1.0 \\
avg (match only)    &  0.9529 &  0.8949 &     1.0 \\
avg (anon*original) &  0.9529 &  0.8949 &     1.0 \\
avg (anon-original) &  0.1502 &  0.1458 &  0.1524 \\
\hline

\end{tabular}
\caption{Re-identification.}
\label{table: Re-identification.}  
\end{table}


\begin{table}[h!]
\centering
\begin{tabular}{| p{4cm} | p{2cm} | p{2cm} | p{2cm} |}

\hline

{} &  RS 20\% &  SS 20\% &    CCSR \\
\hline

words               &     1.0 &     1.0 &     1.0 \\
avg (match only)    &  0.9986 &  0.5486 &  0.7512 \\
avg (anon*original) &  0.9986 &  0.5486 &  0.7512 \\
avg (anon-original) &  0.1518 &  0.1084 &  0.1388 \\
\hline

\end{tabular}
\caption{Re-identification.}
\label{table: Re-identification.}  
\end{table}




\begin{table}[h!]
\centering
\begin{tabular}{| p{4cm} | p{2cm} | p{2cm} | p{2cm} |}

\hline

{} &    Agg2 &    Agg3 &    Agg4 \\
\hline

words               &  0.9063 &  0.6351 &  0.2789 \\
avg (match only)    &  0.5939 &  0.4593 &  0.3915 \\
avg (anon*original) &  0.5758 &  0.4261 &   0.347 \\
avg (anon-original) &  0.1646 &  0.1603 &  0.1531 \\
\hline

\end{tabular}
\caption{Re-identification.}
\label{table: Re-identification.}  
\end{table}





